A Distributed Parallel Optimization Algorithm via Alternating Direction Method of Multipliers

Alternating Direction Method of Multipliers (ADMM) algorithm has been widely adopted for solving the distributed optimization problem (DOP). In this paper, a new distributed parallel ADMM algorithm is proposed, which allows the agents to update their local states and dual variables in a completely distributed and parallel manner by modifying the existing distributed sequential ADMM. Moreover, the updating rules and storage method for variables are illustrated. It is shown that all the agents can reach a consensus by asymptotically converging to the optimal solution. Besides, the global cost function will converge to the optimal value at a rate of O(1/k). Simulation results on a numerical example are given to show the effectiveness of the proposed algorithm.

==> ref.tex <==


@article{zhang2015distributed,
  title={Distributed projection-based algorithms for source localization in wireless sensor networks},
  author={Zhang, Yanqiong and Lou, Youcheng and Hong, Yiguang and Xie, Lihua},
  journal={IEEE Transactions on Wireless Communications},
  volume={14},
  number={6},
  pages={3131--3142},
  year={2015},
  publisher={IEEE}
}

%2
@article{wu2018game,
  title={A game theory based collaborative security detection method for Internet of Things systems},
  author={Wu, Hao and Wang, Wei},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={13},
  number={6},
  pages={1432--1445},
  year={2018},
  publisher={IEEE}
}



@article{zhang2018admm,
  title={ADMM based privacy-preserving decentralized optimization},
  author={Zhang, Chunlei and Ahmad, Muaz and Wang, Yongqiang},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={14},
  number={3},
  pages={565--580},
  year={2018},
  publisher={IEEE}
}

%4

@article{salehisadaghiani2019distributed,
  title={Distributed Nash equilibrium seeking under partial-decision information via the alternating direction method of multipliers},
  author={Salehisadaghiani, Farzad and Shi, Wei and Pavel, Lacra},
  journal={Automatica},
  volume={103},
  pages={27--35},
  year={2019},
  publisher={Elsevier}
}





@article{salehisadaghiani2016distributed,
  title={Distributed Nash equilibrium seeking: A gossip-based algorithm},
  author={Salehisadaghiani, Farzad and Pavel, Lacra},
  journal={Automatica},
  volume={72},
  pages={209--216},
  year={2016},
  publisher={Elsevier}
}


@article{cortes1995support,
  title={Support-vector networks},
  author={Cortes, Corinna and Vapnik, Vladimir},
  journal={Machine learning},
  volume={20},
  number={3},
  pages={273--297},
  year={1995},
  publisher={Springer}
}


@article{boyd2010distributed,
  title={Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers},
  author={Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan},
  journal={Machine Learning},
  volume={3},
  number={1},
  pages={1--122},
  year={2010}
}




@article{yan2020parallel,
  title={Parallel alternating direction method of multipliers},
  author={Yan, Jiaqi and Guo, Fanghong and Wen, Changyun and Li, Guoqi},
  journal={Information Sciences},
  volume={507},
  pages={185--196},
  year={2020},
  publisher={Elsevier}
}


@inproceedings{bazerque2010distributed,
  title={Distributed lasso for in-network linear regression},
  author={Bazerque, Juan Andr{\'e}s and Mateos, Gonzalo and Giannakis, Georgios B},
  booktitle={2010 IEEE International Conference on Acoustics, Speech and Signal Processing},
  pages={2978--2981},
  year={2010},
  organization={IEEE}
}



@article{yang2019survey,
  title={A survey of distributed optimization},
  author={Yang, Tao and Yi, Xinlei and Wu, Junfeng and Yuan, Ye and Wu, Di and Meng, Ziyang and Hong, Yiguang and Wang, Hong and Lin, Zongli and Johansson, Karl H},
  journal={Annual Reviews in Control},
  volume={47},
  pages={278--305},
  year={2019},
  publisher={Elsevier}
}



@article{guo2017hierarchical,
  title={Hierarchical decentralized optimization architecture for economic dispatch: A new approach for large-scale power system},
  author={Guo, Fanghong and Wen, Changyun and Mao, Jianfeng and Chen, Jiawei and Song, Yong-Duan},
  journal={IEEE Transactions on Industrial Informatics},
  volume={14},
  number={2},
  pages={523--534},
  year={2017},
  publisher={IEEE}
}

%12
@article{guo2017distributed,
  title={A distributed hierarchical algorithm for multi-cluster constrained optimization},
  author={Guo, Fanghong and Wen, Changyun and Mao, Jianfeng and Li, Guoqi and Song, Yong-Duan},
  journal={Automatica},
  volume={77},
  pages={230--238},
  year={2017},
  publisher={Elsevier}
}


@article{nedic2009distributed,
  title={Distributed subgradient methods for multi-agent optimization},
  author={Nedic, Angelia and Ozdaglar, Asuman},
  journal={IEEE Transactions on Automatic Control},
  volume={54},
  number={1},
  pages={48--61},
  year={2009},
  publisher={IEEE}
}


@article{nedic2010constrained,
  title={Constrained consensus and optimization in multi-agent networks},
  author={Nedic, Angelia and Ozdaglar, Asuman and Parrilo, Pablo A},
  journal={IEEE Transactions on Automatic Control},
  volume={55},
  number={4},
  pages={922--938},
  year={2010},
  publisher={IEEE}
}


%15
@article{xu2017convergence,
  title={Convergence of asynchronous distributed gradient methods over stochastic networks},
  author={Xu, Jinming and Zhu, Shanying and Soh, Yeng Chai and Xie, Lihua},
  journal={IEEE Transactions on Automatic Control},
  volume={63},
  number={2},
  pages={434--448},
  year={2017},
  publisher={IEEE}
}

%16
@article{duchi2011dual,
  title={Dual averaging for distributed optimization: Convergence analysis and network scaling},
  author={Duchi, John C and Agarwal, Alekh and Wainwright, Martin J},
  journal={IEEE Transactions on Automatic control},
  volume={57},
  number={3},
  pages={592--606},
  year={2011},
  publisher={IEEE}
}

%17
@article{xi2017dextra,
  title={DEXTRA: A fast algorithm for optimization over directed graphs},
  author={Xi, Chenguang and Khan, Usman A},
  journal={IEEE Transactions on Automatic Control},
  volume={62},
  number={10},
  pages={4980--4993},
  year={2017},
  publisher={IEEE}
}


%18
@article{shi2015extra,
  title={Extra: An exact first-order algorithm for decentralized consensus optimization},
  author={Shi, Wei and Ling, Qing and Wu, Gang and Yin, Wotao},
  journal={SIAM Journal on Optimization},
  volume={25},
  number={2},
  pages={944--966},
  year={2015},
  publisher={SIAM}
}


%19
@article{pu2020push,
  title={Push--pull gradient methods for distributed optimization in networks},
  author={Pu, Shi and Shi, Wei and Xu, Jinming and Nedi{\'c}, Angelia},
  journal={IEEE Transactions on Automatic Control},
  volume={66},
  number={1},
  pages={1--16},
  year={2020},
  publisher={IEEE}
}

%20
@article{bauschke1994dykstra,
  title={Dykstra' s alternating projection algorithm for two sets},
  author={Bauschke, Heinz H and Borwein, Jonathan M},
  journal={Journal of Approximation Theory},
  volume={79},
  number={3},
  pages={418--443},
  year={1994},
  publisher={Elsevier}
}


@article{combettes2007douglas,
  title={A Douglas--Rachford splitting approach to nonsmooth convex variational signal recovery},
  author={Combettes, Patrick L and Pesquet, Jean-Christophe},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={1},
  number={4},
  pages={564--574},
  year={2007},
  publisher={IEEE}
}


@inproceedings{wei2012distributed,
  title={Distributed alternating direction method of multipliers},
  author={Wei, Ermin and Ozdaglar, Asuman},
  booktitle={2012 IEEE 51st IEEE Conference on Decision and Control (CDC)},
  pages={5445--5450},
  year={2012},
  organization={IEEE}
}


%23
@article{deng2017parallel,
  title={Parallel multi-block ADMM with O (1/k) convergence},
  author={Deng, Wei and Lai, Ming-Jun and Peng, Zhimin and Yin, Wotao},
  journal={Journal of Scientific Computing},
  volume={71},
  number={2},
  pages={712--736},
  year={2017},
  publisher={Springer}
}


@article{shi2014linear,
  title={On the linear convergence of the ADMM in decentralized consensus optimization},
  author={Shi, Wei and Ling, Qing and Yuan, Kun and Wu, Gang and Yin, Wotao},
  journal={IEEE Transactions on Signal Processing},
  volume={62},
  number={7},
  pages={1750--1761},
  year={2014},
  publisher={IEEE}
}

@book{horn2012matrix,
  title={Matrix analysis},
  author={Horn, Roger A and Johnson, Charles R},
  year={2012},
  publisher={Cambridge university press}
}


%27

@article{nedic2018network,
  title={Network topology and communication-computation tradeoffs in decentralized optimization},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex and Rabbat, Michael G},
  journal={Proceedings of the IEEE},
  volume={106},
  number={5},
  pages={953--976},
  year={2018},
  publisher={IEEE}
}



@inproceedings{mai2016distributed,
  title={Distributed optimization over weighted directed graphs using row stochastic matrix},
  author={Mai, Van Sy and Abed, Eyad H},
  booktitle={2016 American Control Conference (ACC)},
  pages={7165--7170},
  year={2016},
  organization={IEEE}
}


@article{wang2019global,
  title={Global convergence of ADMM in nonconvex nonsmooth optimization},
  author={Wang, Yu and Yin, Wotao and Zeng, Jinshan},
  journal={Journal of Scientific Computing},
  volume={78},
  number={1},
  pages={29--63},
  year={2019},
  publisher={Springer}
}


@inproceedings{wei20131,
  title={On the o (1= k) convergence of asynchronous distributed alternating direction method of multipliers},
  author={Wei, Ermin and Ozdaglar, Asuman},
  booktitle={2013 IEEE Global Conference on Signal and Information Processing},
  pages={551--554},
  year={2013},
  organization={IEEE}
}



@article{nedic2014distributed,
  title={Distributed optimization over time-varying directed graphs},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={60},
  number={3},
  pages={601--615},
  year={2014},
  publisher={IEEE}
}



@article{nedic2016stochastic,
  title={Stochastic gradient-push for strongly convex functions on time-varying directed graphs},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={12},
  pages={3936--3947},
  year={2016},
  publisher={IEEE}
}

%
@article{xi2018linear,
  title={Linear convergence in optimization over directed graphs with row-stochastic matrices},
  author={Xi, Chenguang and Mai, Van Sy and Xin, Ran and Abed, Eyad H and Khan, Usman A},
  journal={IEEE Transactions on Automatic Control},
  volume={63},
  number={10},
  pages={3558--3565},
  year={2018},
  publisher={IEEE}
}


@inproceedings{zhang2014asynchronous,
  title={Asynchronous distributed ADMM for consensus optimization},
  author={Zhang, Ruiliang and Kwok, James},
  booktitle={International conference on machine learning},
  pages={1701--1709},
  year={2014},
  organization={PMLR}
}


@article{he2016proximal,
  title={On the proximal Jacobian decomposition of ALM for multiple-block separable convex minimization problems and its relationship to ADMM},
  author={He, Bingsheng and Xu, Hong-Kun and Yuan, Xiaoming},
  journal={Journal of Scientific Computing},
  volume={66},
  number={3},
  pages={1204--1217},
  year={2016},
  publisher={Springer}
}



@article{simonetto2014distributed,
  title={Distributed maximum likelihood sensor network localization},
  author={Simonetto, Andrea and Leus, Geert},
  journal={IEEE Transactions on Signal Processing},
  volume={62},
  number={6},
  pages={1424--1437},
  year={2014},
  publisher={IEEE}
}

%
